VideoClusterNet: Self-Supervised and Adaptive Face Clustering For Videos

With the rise of digital media content production, the need for analyzing movies and TV series episodes to locate the main cast of characters precisely is gaining importance.Specifically, Video Face Clustering aims to group together detected video face tracks with common facial identities. This problem is very challenging due to the large range of pose, expression, appearance, and lighting variations of a given face across video frames. Generic pre-trained Face Identification (ID) models fail to adapt well to the video production domain, given its high dynamic range content and also unique cinematic style. Furthermore, traditional clustering algorithms depend on hyperparameters requiring individual tuning across datasets. In this paper, we present a novel video face clustering approach that learns to adapt a generic face ID model to new video face tracks in a fully self-supervised fashion. We also propose a parameter-free clustering algorithm that is capable of automatically adapting to the finetuned model's embedding space for any input video. Due to the lack of comprehensive movie face clustering benchmarks, we also present a first-of-kind movie dataset: MovieFaceCluster. Our dataset is handpicked by film industry professionals and contains extremely challenging face ID scenarios. Experiments show our method's effectiveness in handling difficult mainstream movie scenes on our benchmark dataset and state-of-the-art performance on traditional TV series datasets.

==> 06.implementation.tex <==
\section{Implementation Details} \label{sec:implementation}

%We discuss finer details of our proposed idea in this section, including model architecture, finetuning procedure etc.    

\subsection{Model Architecture}
\label{appendix:arch_details}
As part of our method, any CNN or Transformer architecture can be incorporated as the base Face ID model. For the attached MLP head, we incorporate a 3-layer network with GELU activation \cite{hendrycks2016_gaussian}. The length of the head's output feature embedding is kept the same as the base model's embedding length. Unnormalized model output embeddings are used for both training and the final clustering stage. Also, teacher branch head weights are initialized separately from their student counterpart. When using a transformer class base model, the head is shared between the class and path token embeddings in both student and teacher branches respectively (\cref{fig:ssl_finetuning}).

\subsection{Data Pre-Processing}
\label{appendix:data_preprocesing_details}
Generation of tracks as part of given video dataset curation for finetuning and/or clustering purposes involves processing the video through the four stage pipeline mentioned in detail in \cref{subsec:track_preprocessing}. To further augment variations in a sampled face crop pair, 'global' and 'local' views are created from the original crops. Specifically, crops are randomly resized and cropped with a scale between 0.7 and 1.0 to create multiple global crops, while a scale between 0.4 and 0.6 provides local crop variants.
Given a total of 6 views for each non-cropped original pair, we set the global and local crop count to 2 and 4, respectively.
%We set the global and local crop count to 2 and 4, for a total of 6 views for each base crop pair.
The loss for a given non-cropped original pair is computed using all possible pairs within each global and local crop group separately. We further apply horizontal flipping and color temperature variations as additional augmentations.  

Face alignment is performed for each face crop prior to the model finetuning and final clustering stages, in order to further enhance model learning of facial features and in turn for better face clustering performance. For this, a given face crop is first resized to the pre-trained model's expected input image size. Then, five point face landmarks are predicted for that crop (we incorporate the landmarks provided as an auxiliary output by the face detection model RetinaFace \cite{deng2020_retinaface} as we empirically find them to be quite accurate). Given the facial landmarks, a similarity transform is computed w.r.t. a mean landmark template. An affine warp is then computed to align the face within the face crop. 

\subsection{Model Finetuning}
\label{appendix:finetuning_details}
For the initial finetuning iteration, we train the model for 30 epochs. Note that the first 10 epochs are dedicated to finetuning the branch heads. All subsequent iterations include 10 training epochs without individual head training stages since the heads aren't randomly reinitialized for every new iteration. The teacher branch weights are updated with the exponential moving average of the student branch weights after every epoch. We adopt AdamW optimizer \cite{Loshchilov2019_decoupled} and an initial learning rate (lr) of $1 \times 10^{-4}$. We use cosine decay scheduling and reduce the lr to a final value of $1 \times 10^{-5}$. The initial lr is linearly warmed up for the first 5 epochs for each iteration from a starting value of $5 \times 10^{-6}$. Experiments were conducted using a Nvidia A10 GPU with 24 GB VRAM, running CUDA 12.0, with code implemented in PyTorch 1.13 \cite{Paszke2019_pytorch}. For finer details on the loss function and training hyperparameters, please refer to \cite{zhou2021_ibot}.

